EvoSchema: Towards Text-to-SQL Robustness Against Schema Evolution

Neural text-to-SQL models, which translate natural language questions (NLQs) into SQL queries given a database schema, have achieved remarkable performance. However, database schemas frequently evolve to meet new requirements. Such schema evolution often leads to performance degradation for models trained on static schemas. Existing work either mainly focuses on simply paraphrasing some syntactic or semantic mappings among NLQ, DB and SQL, or lacks a comprehensive and controllable way to investigate the model robustness issue under the schema evolution, which is insufficient when facing the increasingly complex and rich database schema changes in reality, especially in the LLM era. To address the challenges posed by schema evolution, we present EvoSchema, a comprehensive benchmark designed to assess and enhance the robustness of text-to-SQL systems under real-world schema changes. EvoSchema introduces a novel schema evolution taxonomy, encompassing ten perturbation types across columnlevel and table-level modifications, systematically simulating the dynamic nature of database schemas. Through EvoSchema, we conduct an in-depth evaluation spanning different open source and closed-source LLMs, revealing that table-level perturbations have a significantly greater impact on model performance compared to column-level changes. Furthermore, EvoSchema inspires the development of more resilient text-to-SQL systems, in terms of both model training and database design. The models trained on EvoSchema's diverse schema designs can force the model to distinguish the schema difference for the same questions to avoid learning spurious patterns, which demonstrate remarkable robustness compared to those trained on unperturbed data on average. This benchmark offers valuable insights into model behavior and a path forward for designing systems capable of thriving in dynamic, real-world environments.

==> review_shepherd.tex <==
\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Shepherd - Page 1}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer_shepherd}{orange color for shepherd}.\\

\textbf{\#\#\# Suggestion}: \\

1. From Table 5, it is noted that models trained with perturbed data (``w/") frequently achieve lower execution accuracy (EX) than those trained without perturbed data (``w/o"), particularly for simpler column-level perturbations (e.g., column addition, deletion, and renaming). Although you have explained that minor decreases fall within an acceptable range, the reviewer would request you to systematically quantify this phenomenon and discuss in more detail. \\


\textbf{\#\#\# Response}: \\

Thanks for the wonderful suggestion! To better understand why training with perturbed data slightly underperforms than training without perturbed data under simpler column-level perturbations, we conducted a detailed error analysis and case studies. We identified two primary types of errors that lead to the phenomenon: \\
\textbf{(1) Spurious or missing conditions in the WHERE clause.} \\
For a question ``What is the element with the atom ID of TR004\_7 in molecule that is not carcinogenic?", the gold SQL is \uline{``SELECT T1.element FROM atom AS T1 INNER JOIN molecule AS T2 ON T1.molecule\_id = T2.molecule\_id WHERE T1.atom\_id = 'TR004\_7' AND T2.label = '-'"}. The model trained with perturbed data predicts a SQL that lacks a condition T2.label = '-' while the model trained without perturbed data can still generate this condition. For a question ``How many transactions were paid in CZK in the morning of 2012/8/26?", the gold SQL is \uline{``SELECT COUNT(T1.TransactionID) FROM transactions\_1k AS T1 INNER JOIN customers AS T2 ON T1.CustomerID = T2.CustomerID WHERE T1.Date = '2012-08-26' AND T1.Time < '13:00:00' AND T2.Currency = 'CZK'"}. The model trained with perturbed data adds a spurious condition "T1.TransactionID BETWEEN 1 AND 1000" in the WHERE clause, while the model trained without perturbed data doesn't add this. 


\textbf{(2) Incorrect column selection in SELECT or WHERE clauses.} \\
For a question ``Among the patients followed at the outpatient clinic, how many of them have a normal level of alkaliphophatase?", the gold SQL is      \uline{``SELECT COUNT(T1.ID) FROM Patient AS T1 INNER JOIN Laboratory AS T2 ON T1.ID = T2.ID WHERE T2.ALP < 300 AND T1.Admission = '-'"}. The model trained with perturbed data can mispredict T1.Admission with T1.Description while the model trained without perturbed data can still correctly select the correct column. For a question ``Which group does superhero A-Bomb belong to?", the gold SQL is \uline{``SELECT T2.race FROM superhero AS T1 INNER JOIN race AS T2 ON T1.race\_id = T2.id WHERE T1.superhero\_name = 'A-Bomb'"}, the model trained with perturbed data wrongly predicts T2.race with another column 'team\_affiliation', while the model trained without perturbed data can still correctly generate the prediction. \\
The above analysis shows that the perturbation augmented training data may introduce minor
noise in simpler schema changes. When schema perturbations are too simple (e.g., adding, removing or renaming columns), the model trained on unperturbed data may have already generalized well to handle such cases. Now, when we introduce perturbed training data, the model sees more diverse variations but some maybe unnecessary, which can distract the model a bit. Some perturbations might conflict slightly with patterns learned from clean unperturbed data, especially if the perturbation introduces edge cases such as 
 spurious or less informative columns. \\

\textbf{\#\#\# Revised Section}: \\

We have added the case studies and corresponding analysis to the Section \ref{main_results} (Main Results).\\

}
\end{tcolorbox}
\end{figure*}



\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Shepherd - Page 2}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer_shepherd}{orange color for shepherd}.\\

\textbf{\#\#\# Suggestion}: \\

2. In the GPT and CHESS experiments in Section 6.1, due to the cost consideration, you only evaluated 50 data samples per perturbation type, which is likely insufficient to ensure statistical significance and hence may significantly reduce the reliability of the experimental findings. Please provide a discussion on this in the paper, and possibly rerun with more data samples. \\

\textbf{\#\#\# Response}: \\

% When we evaluated 50 examples for each perturbation type, we still have 500 examples in total for each baseline. To demonstrate the effectiveness of our method (train w/ perturbation data), we
% perform McNemar’s Test \citep{} to measure the statistical significance on each baseline with our method (trained w/ perturbation data) to measure the statistical significance of our method. For each significance test between two methods, we use we compute the
% p-values using statsmodels. When p < 0.05, we reject the null hypothesis. In other words, we consider the accuracy improvement statistically significant when p < 0.05. By McNemar’s test, we find that our method can achieve statistically significant improvement over three baselines: GPT4 in context learning, finetuning w/o perturbation data and CHESS (p < 0.05). 
% To further enhance the reliability of our experiments, we increase sample size from 50 to 200 for each perturbation type, i.e., from 500 to 2000 for each baseline and our method to demonstrate findings. Our experiments show that our previous findings still hold.

% To evaluate the effectiveness of our method (training with perturbed data), we initially sampled 50 examples per perturbation type, totaling 500 examples for each baseline. We conducted McNemar’s Test \citep{mcnemar1947note} to assess the statistical significance of accuracy improvements when comparing our method against each baseline. For each pairwise comparison, we computed p-values using the statsmodels package. A result is considered statistically significant when p < 0.05, meaning we reject the null hypothesis and interpret the observed improvement as unlikely to be due to chance. 

% Using McNemar’s Test, we found that our method achieves statistically significant improvements over three key baselines: GPT-4 in-context learning, fine-tuning without perturbed data, and CHESS (p < 0.05 in each case). 

% To further enhance the reliability of our results, we expanded the evaluation to 200 examples per perturbation type—scaling the total from 500 to 2000 examples per method. The updated experiments confirm that our original findings remain consistent and robust at larger scale. \\
To assess the effectiveness of our method (training with perturbed data), previously we evaluated 50 examples per perturbation type, resulting in 500 total examples per method. We applied McNemar’s Test \citep{mcnemar1947note} to measure the statistical significance of performance differences between our method and each baseline. We computed p-values using the \texttt{statsmodels} package, considering differences statistically significant when 
$p<0.05$, which indicates that the improvement is unlikely due to random chance.

Using this test, we observed our method achieved statistically significant improvements over three key baselines: GPT-4 in-context learning, fine-tuning without perturbed data, and CHESS (all with $p<0.05$).

To further strengthen the reliability of our findings, we increased the evaluation sample size to 200 examples per perturbation type, scaling the total to 2,000 examples per method. The updated results is shown in Table~\ref{tab:bird_human_eval} and confirm that the original findings are consistent and robust at a larger scale. \\

\textbf{\#\#\# Revised Section}: \\
We have updated Table~\ref{tab:bird_human_eval} and Section~\ref{baseline_comparison} to reflect the expanded evaluation from 50 to 200 examples per perturbation type. \\

\textbf{\#\#\# Suggestion}: \\

3. For table merge and split perturbations, approximately 100 hours of manual effort were incurred to correct the gold SQL annotations. This manual requirement highlights a significant limitation of the approach regarding automation, which is unacceptable for a new benchmark. \\

\textbf{\#\#\# Response}: \\

The manual efforts mentioned by the reviewer was for curating the evaluation data, not the training data. As with any benchmark, this one-time effort ensures the accuracy and reliability of evaluation results, allowing the broader community to use the data without repeating the verification process. In contrast, our training data is generated entirely automatically without any human annotation or manual verification. We believe the reviewer may have been referring to training data generation, in which case we would like to clarify that our approach is fully automated in that regard. 

Moreover, the manual efforts required for our evaluation benchmark is already substantially lower compared to prior benchmarks, enabled by our automated data generation framework. For instance, the widely used Spider dataset \cite{yu-etal-2018-spider} reports approximately 1000 hours of manual data collection effort, which is nearly 10 times more than what was needed for our human verification cost.

If our methodology were to be extended to other datasets, the amount of manual effort required would depend on the complexity of the schema, the quality of LLM-generated perturbations and the dataset size. Besides, as the LLMs' ability become more and more stronger, in future work, we also envision leveraging LLM-based evaluators (e.g., LLM-as-a-Judge) to further reduce or eliminate the need for manual correction, though that is beyond the scope of this paper. \\

\textbf{\#\#\# Revised Section}: We have updated the Cost Analysis in Section~\ref{cost_analysis} to clarify this distinction. \\

}
\end{tcolorbox}
\end{figure*}




% \begin{figure*}[htbp]
% \begin{tcolorbox}
% [colback=white, colframe=gray!60!black,
% title={\huge Shepherd - Page 3}, fontupper=\footnotesize, fonttitle=\footnotesize]
% {\Large

% We mark the relevant revision part in the paper using \textcolor{reviewer_shepherd}{orange color for shepherd}.\\

% \textbf{\#\#\# Suggestion}: \\

% 3. For table merge and split perturbations, approximately 100 hours of manual effort were incurred to correct the gold SQL annotations. This manual requirement highlights a significant limitation of the approach regarding automation, which is unacceptable for a new benchmark. \\

% \textbf{\#\#\# Response}: \\

% We believe there may be a misunderstanding. The manual effort cited by the reviewer was solely for curating the evaluation data, not the training data. As with any benchmark, this one-time effort ensures the accuracy and reliability of evaluation results, allowing the broader community to use the data without repeating the verification process.

% In contrast, our training data is generated automatically without any human annotation or manual verification. We believe the reviewer may have been referring to training data generation, in which case we would like to clarify that our approach is fully automated in that regard.

% If our methodology were to be extended to other datasets, the amount of manual effort required would depend on the complexity of the schema and the quality of LLM-generated perturbations, which may vary by model. In future work, we also envision leveraging LLM-based evaluators (e.g., LLM-as-a-judge) to further reduce or eliminate the need for manual correction—though that is beyond the scope of this paper.


% % I feel there should be some misunderstanding for the reviewer. If people need our evaluation data, then our time is just one-time effort: we ensure the quality and people can use it. This process is needed for any benchmark. But for automation part, which means the training data generation, we don't have manual human verification. I think the reviewer refers to the latter but we actually don't spend time verifying training data. 

% % if the goal is to apply to other datasets, the manual effort needed depends on what LLM is used and how complex the dataset is, that could have an impact on the quality of LLM generated perturbation, it could be the case that the effort needed is lower.
% % we can also explore using LLM-judge to facilitate the correction, but this can be future work and it out of scope for this paper. \\

% \textbf{\#\#\# Revised Section}:

% We have updated the Cost Analysis in Section~\ref{cost_analysis} to clarify this distinction. \\

% }
% \end{tcolorbox}
% \end{figure*}


\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Shepherd - Page 3}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer_shepherd}{orange color for shepherd}.\\

\textbf{\#\#\# Suggestion}: \\

4. recent surveys and empirical studies have also addressed the schema problem; please discuss them carefully in the related work section [a][b].

[a] Liu, Xinyu, et al. "A Survey of NL2SQL with Large Language Models: Where are we, and where are we going?." arXiv preprint arXiv:2408.05109 (2024).

[b] Li, Boyan, et al. "The dawn of natural language to SQL: are we fully ready?." PVLDB(2024). \\

\textbf{\#\#\# Response}: \\

% Our Table \ref{tab:comparison_with_existing_benchmarks}, Section \ref{related_work} (Related Work) and Section \ref{comparison_with_existing_benchmarks} (Comparison with Existing Benchmarks) have already discussed the details or the most relevant schema evolution work that align with our problem such as  DrSpider, ADVETA, MT-TEQL and our EvoSchema. While the reviewer mention the two surveys, they are not specically address the schema evolution problem that very slimilar with ours. They provide a more broader overview and lifecycle of text-to-SQL problems. For [a], they systematically review the entire lifecycle of NL2SQL problem which cover four aspects: nl2sql models, benchmarks and data synthesis, evaluation and error analysis. Our main contribution is to explore how the recent advanced LLMs robust to different schema evolution problem. From the model perspective, we mainly
% evaluate more recent and powerful LLMs, including fine-tuning advanced open-source models (CodeLlama,
% Mistral, SQLCoder, LLaMA 3) and prompting closed-source models (GPT-3.5, GPT-4). These recent models
% can be used without preprocessing or postprocessing steps for SQL generation and are still under-explored. For the benchmark and training data synthesis perspective, we build our evaluation benchmark with systematic schema perturbation types, and evaluate the NL2SQL robustness through this unique angle. Based on this angle, we also synthesize our training data in this more structured way. From the evaluation pespective, we not only use execution accuracy and human evaluation, but also propose two new metrics: table match F1 and column match F1 to have a more fine-grained evalution to study the column selection and table selection during SQL generation, which  highly echos our schema evolution taxonomy: column-level and table-level perturbation. 
 
% For [b], they evaluate different prompting closed-source models and finetuning open-source LLMs. However, their examperimets are done on Spider and BIRD raw dataset, while in our work, we first build the suitable benchmark to cover different schema variations and then do the experiments on both the original BIRD dataset and our different perturbed evaluation set. Besides, they have a Query Variance Testing experiment, which is to test the existing NL2SQL solutions' performance against NL variations, where for the same SQL, they have different variations of their natural language quesiton. In our work, our variation is done on the database schema, while we keep the natural lauguage the same.


Our Table~\ref{tab:comparison_with_existing_benchmarks}, Section~\ref{related_work} (Related Work), and Section~\ref{comparison_with_existing_benchmarks} (Comparison with Existing Benchmarks) already provide a detailed discussion of prior work most relevant to our schema evolution problem, including DrSpider, ADVETA, MT-TEQL, and FootballDB. While the reviewer highlights a recent survey [a] and a study [b], we note that these two work offer broader overviews of the NL2SQL landscape rather than directly addressing the schema evolution challenges that our work focuses on.

Survey [a] systematically reviews the entire NL2SQL lifecycle across four dimensions: NL2SQL models, benchmarks and training data synthesis, evaluation, and error analysis. Our focus is more specific: the NL2SQL robustness against schema evolution - a problem they identify but do not explore in depth.  From the model perspective, we mainly evaluate more recent and powerful LLMs, including fine-tuning advanced open-source models (Code Llama, Mistral, SQLCoder and LLaMA 3) and prompting closed-source models (GPT-3.5, GPT-4). These recent models can be used without preprocessing or postprocessing steps for SQL generation and are still under-explored. From the benchmark and data synthesis perspective, we introduce \texttt{EvoSchema}, a systematic taxonomy featuring controlled schema perturbations. This enables us to study NL2SQL model robustness from a schema-centric angle, which also enables the structured synthesis of our training data. From the evaluation perspective, we not only use standard execution accuracy and human evaluation, but also introduce two fine-grained metrics: Table Match F1 and Column Match F1. These metrics allow us to study the column selection and table selection during SQL generation, which closely aligns with our taxonomy of column-level and table-level perturbations.

Study [b] evaluates both prompted closed-source and fine-tuned open-source LLMs but conducts all experiments on unperturbed datasets (Spider and BIRD). In contrast, our work constructs a benchmark specifically designed to test model robustness against different schema evolution types and then conducts experiments on both the original and perturbed versions of BIRD. Moreover, [b] conducts a query variance testing experiment, which investigates robustness against natural language variations for a fixed SQL query. Our focus is orthogonal: we evaluate robustness against schema variations while keeping the natural language question fixed. \\

% In summary, while [a] and [b] provide valuable context, our work complements them by offering a focused and deeper investigation into schema evolution—an important, yet under-explored, dimension of NL2SQL robustness.

\textbf{\#\#\# Revised Section}: \\

We have added the discussion to the  Section \ref{related_work} (Related Work).
}
\end{tcolorbox}
\end{figure*}


==> reviewer1.tex <==
% \begin{center}
%     {\huge General Comments} \\
% \end{center}


% {\large
% 1. We have addressed the great majority of the suggestions from the reviewers. Only a few
% suggestions that could not be addressed have been properly justified;\\

% 2. We have performed more experiments encompassing a new dataset;\\

% 3. We have performed more experiments to present the sensitivity analysis of the
% parameters employed by our approach; \\

% 4. Following the suggestions of the reviewers, we have improved many sections of the article
% by pointing out other related works, adding new examples, discussing the results in more
% details and presenting lessons learned from the obtained experimental results; \\

% 5. We have highlighted in blue the sentences and results added to the new version of our
% manuscript; \\

% 6. We would like to extend our sincere gratitude for the detailed and constructive feedback
% provided on our manuscript. Your insights and suggestions have been invaluable and have
% significantly contributed to improving the quality and clarity of our work. The following tables
% list these suggestions in addition to the respective justifications or solutions implemented. \\
% }


\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Reviewer 1 - Page 1}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer1}{red color for reviewer 1}. Note execution accuracy results are marked as \textcolor{reviewer3}{green} in Table \ref{tab:bird_exec_acc}.\\

\textbf{\#\#\# Suggestion}: \\

The paper should be compared to the following paper, which also studied the problem of schema evolution and provided a benchmark dataset on real queries where both the train and the test data reflect schema changes:

[1] Jonathan Fürst, Catherine Kosten, Farhad Nooralahzadeh, Yi Zhang, Kurt Stockinger: Evaluating the Data Model Robustness of Text-to-SQL Systems Based on Real User Queries. EDBT 2025: 158-170 \\

\textbf{\#\#\# Response}: \\

We compare our work with theirs from the following four perspectives: \\
(1) Motivation: 

[1] explores three manually designed schema versions for a single Football database, aiming to identify a schema that is beneficial for SQL writing. Their first evolution (v1 → v2) addresses 1:N foreign key mappings, which can complicate pre-/post-processing in some text-to-SQL models. However, this also increases the number of tables and required joins. So their second evolution (v2 → v3) is to reduce the JOIN complexity. In contrast, our work takes a different view of schema evolution. Schema evolution is driven not only by structural reorganization (e.g., splitting or merging tables), but also by the need to incorporate new information (e.g., adding columns or tables), and we analyze how these changes affect NL2SQL performance.
% In contrast, our work focuses on schema evolution more broadly, motivated by practical needs not only for schema reorganization such as splitting and merging tables, but also considering how new information required the scheme change such as adding columns or tables, and investigates how such changes impact NL2SQL performance.

(2) Schema Evolution Types:

While [1] focuses primarily on reducing PK/FK references and minimizing JOIN complexity, our work explores the schema evolution from a different angle, where we introduce a more comprehensive and systematic taxonomy of schema evolution types. We analyze both table-level and column-level changes, including adding, removing, renaming, splitting, and merging columns and tables and aim at offering a broader and more structured exploration of schema evolution.

(3) Model Scope:

[1] includes earlier models like ValueNet and PICARD, which rely on pre- and post-processing. We mainly evaluate more recent and powerful LLMs, including fine-tuning advanced open-source models (CodeLlama, Mistral, SQLCoder, LLaMA 3) and prompting closed-source models (GPT-3.5, GPT-4). These recent models can be used without preprocessing or postprocessing steps for SQL generation and are still under-explored. 

(4) Data Scale and Generalizability:

[1] evaluates on three manually curated schema versions of a single Football database. In contrast, our work builds on BIRD, a complex, realistic multi-database benchmark. Our framework enables systematic schema evolution across multiple databases, providing more scalable and generalizable experimental results. This directly addresses a limitation in [1], which is confined to a single-domain, single-database setting. \\


% (1) From the motivataion perspective, their work explores three versions of designed schema for their proposed Football database and tries to find a better database schema design that is beneficial for SQL writing. For their first evolution from design v1 to design v2, the motivation of this evolution is to address the 1:N foreign key mappings between tables, which will cause issues during the pre-processing or post-processing stage for several text-to-SQL models. From design v1 to design v2, there are more tables in the database, and the SQL query needs to join more tables. Our work focuses on scheme evolution, which not only covers database schema reorganization, but inspired by when new information come will need us to revise the existing database design such as add columns, add tables. and want to explore how these change will affect the NL2SQL performance. \\
% (2) From the scheme evolution types perspective, [1] mainly revise their schema design to reduce PK/FK references among tables and reduce JOIN paths for SQL queries. while our work mainly try to give a more comprehensive, systematic and structured taxonomy and analysis for different schema evolution types. Instead of just analyzing these two specific types, we systematically build a taxonomy to explore the table-level and column-level schema evolution that covers more comprehensive types such as adding/removing/renaming/splitting/merging tables and columns. \\
% (3) From the model perspective, we mainly explore the more advanced open-sourced models (codellama, mistral, sqlcoder and llama3) and closed-sourced models (gpt-3.5 and gpt-4). The ValueNet and Picard in their work are relatively older models that still require pre-processing and post-processing steps. As the more advanced open-sourced models have emerged recently and are much more powerful than the models selected by [1], we consider that our selected advanced models are still under-explored for this schema evolution problem and are more convenient which don’t require pre-processing and post-processing. \\
% (4) From the data scale perspective, [1] only three manually designed versions of the schema and the schema is within the same database. Our work builds our dataset based on a complex, realistic and multiple-database dataset: BIRD. We provide the framework that allows us to systematically get different versions of the schema under more comprehensive schema evolution types and apply it on different databases in BIRD instead of just a single Football database. So our analysis is based on multiple databases and provides more reliable quantitative results and our findings will be more generalizable, which can address the limitation mentioned in [1], that they only do experiments on a single database dataset. \\

\textbf{\#\#\# Revised Section}: \\

We add this work into Table \ref{tab:comparison_with_existing_benchmarks} to compare with other schema perturbation related work: DrSpider, ADVETA, MT-TEQL and our EvoSchema. Besides, we also revise the Section \ref{related_work} (Related Work) and Section \ref{comparison_with_existing_benchmarks} (Comparison with Existing Benchmarks) to compare this work.

% \noindent\rule{\linewidth}{0.5pt}

}
\end{tcolorbox}
% \caption{\textbf{Schema augmentation} task. This task is to populate the possible headers for a table, given the table caption and the seed table header.}
% \label{fig:schema_aug}
\end{figure*}


\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Reviewer 1 - Page 2}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer1}{red color for reviewer 1}. Note execution accuracy results are marked as \textcolor{reviewer3}{green} in Table \ref{tab:bird_exec_acc}.\\\

\textbf{\#\#\# Suggestion}: \\

In general, the experiments need to be better described and be modelled in a more realistic setting where both the schema and the queries evolve over time. It is unrealistic that the schema evolves over time and the testing is done on non-evolved schema. In other words, the test set queries should be extended with new queries against evolved schema. \\

\textbf{\#\#\# Response}: \\

We want to clarify that the reviewer misunderstood our experiment design. We indeed adopted the reviewer-mentioned realistic setting and designed the experiment to let both the schema and SQL queries evolve over time. And for both training data and test data, we included new schema and new queries against evolved schema. As the second paragraph (Schema Perturbations) in Section \ref{seed_data_select} (Seed Dataset Selection) in the paper mentioned, we apply the schema evolution on the entire BIRD dataset and get both the new schema and new SQL queries. The train/test split examples are aligned with the original BIRD train/dev split. Table~\ref{tab:data_stat_plus_manipulated_stat} presents the data statistics used in our experiments. ``Original'' refers to the raw BIRD training and evaluation data without any schema evolution. While other rows show each schema evolution type, and we report the corresponding training and evaluation statistics. Here, ``eval" denotes the test set, which includes both evolved schemas and new queries. In Table \ref{tab:bird_main_results2}, the row labeled ``Original" reports performance on the original BIRD test set (no schema evolution), while the other rows (e.g., add columns) show results on test sets where both the schema and queries have been modified. For each model (e.g., CodeLlama, Mistral, Llama3 and SQLCoder), there are two columns to show the results. w/o column indicates the model is trained without perturbation training data, while w/ column indicates the model is trained with perturbation data. For both trained w/o and w/ perturbation training data, we evaluate them on non-evolved (Original) test set and each type of evolved test set.  \\


\textbf{\#\#\# Highlighted Section}: \\

We highlight how we prepare our train/eval data for both non-evolved and evolved sets. Please check `Schema Perturbations' in Section \ref{seed_data_select} (Seed Dataset Selection) in the paper.

Please check Table \ref{tab:bird_main_results2} and Table \ref{tab:bird_exec_acc} for results on both the non-evolved test set and evolved test set. Note: for each model (e.g., CodeLlama, etc), w/o column indicates the model is trained without perturbation train data, while w/ column indicates the model is trained with perturbation train data. For both trained w/o and w/ perturbation train data, we evaluate them on non-evolved (Original) test set and each type of evolved test set. \\

\noindent\rule{\linewidth}{0.5pt}

\textbf{\#\#\# Suggestion}: \\

It seems that the test data is the same whereas the training used is without and with perturbations. It would be important to add new test queries that are executed against the schema that evolved over time. \\

\textbf{\#\#\# Response}: \\

As mentioned above, our test setting includes both non-evolved and evolved queries. The non-evolved queries come from the original BIRD dev set, while the evolved queries are generated by applying ten schema evolution types to the original BIRD dev set. Similarly, the training set includes both the original (non-evolved) BIRD training data and the corresponding evolved versions.\\




}
\end{tcolorbox}
\end{figure*}


\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Reviewer 1 - Page 3}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer1}{red color for reviewer 1}. Note execution accuracy results are marked as \textcolor{reviewer3}{green} in Table \ref{tab:bird_exec_acc}.\\\

\textbf{\#\#\# Suggestion}: \\

The evaluation needs to be improved. Table 3 shows the F1 score of table match for various LLMs but no execution accuracy. Table 4 only shows execution accuracy, but it is not clear for which LLM. \\

\textbf{\#\#\# Response and Revised Section}: \\


We add Table \ref{tab:bird_exec_acc} to show the execution accuracy for all the LLMs (CodeLlama, Mistral, Llama3, SQLCoder, GPT-3.5 and GPT4) mentioned in Table \ref{tab:bird_main_results2}. And also we add human evaluation results in Table \ref{tab:bird_human_eval}. \\


\noindent\rule{\linewidth}{0.5pt}

\textbf{\#\#\# Suggestion}: \\

The authors write “Since the NLQs are the same for adding or removing columns and tables”. This is not correct. When you remove columns and tables, existing NLQs might not work anymore. \\

\textbf{\#\#\# Response}: \\

When we apply removing columns and tables perturbations, we detect whether the gold SQL contains the columns or tables that will be removed. If yes, then the corresponding NLQs don't work, and we will change our ground truth for these NLQs as ``The table/column information is not enough for generating the SQL query to answer the question.'' We show our experiments in Section \ref{out_of_scope_exp} (Influence of Out-of-scope Types). If these removed tables and columns aren't included in the gold SQL, then these NLQs still work, and we can still examine how they will influence the SQL generation for these NLQs. \\


\noindent\rule{\linewidth}{0.5pt}

\textbf{\#\#\# Suggestion}: \\
The authors write “Add tables: We randomly add irrelevant tables to each question, and these tables are still in the same database as the relevant tables in BIRD. [..] The tables added don’t affect the NLQ and the gold SQL”. It is not clear why you want to add random tables in the SQL without affecting the NLQ. Can you give concrete example to 
justify this from a real-world perspective? \\


\textbf{\#\#\# Response}: \\


Thank you for your thoughtful question. Our goal in adding irrelevant tables is to simulate real-world scenarios where databases often contain many tables unrelated to a given user query. In such settings, a robust text-to-SQL model must be able to identify and focus on the relevant subset of the schema while ignoring distracting or unrelated tables.

For example, in a university database with tables such as Students, Courses, and Enrollments, a user may ask: “What are the names of students enrolled in CS101?” Although the correct SQL query only involves the three aforementioned tables, the full schema may also include tables like DormRooms or CafeteriaMenus, which are unrelated to the question. In this case, the model is expected to ignore these irrelevant tables and still generate the correct SQL. Our perturbation ``add tables'' intentionally mimics this setting by introducing such extraneous tables, without changing the NLQ or the gold SQL, in order to evaluate the model’s ability to remain focused and accurate in the presence of schema distraction.






}
\end{tcolorbox}
\end{figure*}



\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Reviewer 1 - Page 4}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer1}{red color for reviewer 1}. Note execution accuracy results are marked as \textcolor{reviewer3}{green} in Table \ref{tab:bird_exec_acc}.\\\

\textbf{\#\#\# Suggestion}: \\

When you split and merge tables, do you make sure that the properties of the three database normal forms are kept? \\


\textbf{\#\#\# Response}: \\

Thank you for the insightful question. While our primary focus is on simulating realistic schema evolution scenarios through table splits and merges, we take care to preserve the principles of the first three normal forms (1NF–3NF) as much as possible.

For table splitting, we ensure that: each resulting table maintains atomic values (1NF); non-key attributes depend on the full pimary key (2NF). And we avoid introducing transitive dependencies (3NF) by separating attributes that do not belong together functionally. For example, when splitting a table that combines student and course enrollment data, we create separate Students, Courses, and Enrollments tables, each with clearly defined primary keys and no redundant or derived attributes.

For table merging, we carefully monitor functional dependencies. But we admit that there is a risk that might introduce non-key to non-key dependencies unintentionally, especially when we merge too much descriptive data into one table. So there is a risk that it might violate 3NF.


 Overall, while our benchmark explores structural variations through schema evolution, we make an effort to preserve the principles of database normalization. \\



\noindent\rule{\linewidth}{0.5pt}



\textbf{\#\#\# Suggestion}: \\

The authors write “We randomly choose 200 generated examples to do manual review and reveal that GPT-3.5 demonstrates a strong understanding of the input context, effectively generating names that meet our requirement”. Can you quantify this better? What is the accuracy of these 200 queries? How do you evaluate the accuracy of other queries that are not manually verified? \\



\textbf{\#\#\# Response}: \\

Thank you for the question. We primarily use GPT-3.5 to rename column/table names or add new columns to the database schema. For SQL queries, we update the gold SQL by replacing original names with the GPT-3.5-generated ones based on the schema changes. So the key is to make sure GPT-3.5 can generate column names or table names correctly. To ensure name generation quality, we randomly sampled 200 examples and found that 94\% of them met our requirements. This automated approach is applied only to add columns, rename columns, and rename tables cases. For more complex schema evolution types, such as split and merge tables, manual verification is still required.

}
\end{tcolorbox}
\end{figure*}

% Thanks for the question. We mainly use GPT-3.5 to rename column/table names, or add column names into the database schema. For SQL queries, we will based on the schema name change to replace the original name in the gold SQL query to the new SQL query. So the key is to make sure GPT-3.5 can generate column names or table names correctly. We randomly select 200 examples and analyze whether the GPT-3.5 generated names meet our requirement. We found that there are 94\% examples can meet our requirements. We only do this for adding columns, renaming columns and renaming tables types. For other more complex schema evolution types like splitting or merging tables, we do need mannully verification.




==> reviewer2.tex <==


\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Reviewer 2 - Page 1}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer2}{blue color for reviewer 2}.\\


\textbf{\#\#\# Suggestion}: \\

 I believe authors are primarily targeting finetuning. Most recent approaches include some in-context learning where the LLM is conditioned to produce SQL, given database schema. I believe in this case database schema evolution would be not an issue. Can authors clarify?\\


\textbf{\#\#\# Response}: \\

We include additional experiments to demonstrate that in-context learning (ICL) alone cannot fully address schema evolution issues. To evaluate its effectiveness, we randomly select three examples (each consisting of an <NLQ, database schema after evolution, gold SQL after schema evolution> triple) as demonstrations in the prompt to help the model understand schema changes. As shown in Table~\ref{tab:bird_human_eval}, ICL significantly outperforms GPT-4 in the zero-shot (ZS) setting only on the split columns perturbation, while offering comparable results for other types. This suggests that ICL is not consistently effective for handling schema evolution. We hypothesize this is because the demonstration examples cannot cover the full diversity of schema and SQL changes; thus, ICL offers limited benefits when test cases differ significantly from the demonstrations. In contrast, split columns often involve predictable patterns (e.g., splitting names, addresses, or dates), making it easier for ICL to generalize. Additionally, Table~\ref{tab:bird_human_eval} shows that fine-tuning CodeLlama with perturbation training data yields better results than ICL on average, indicating that fine-tuning with perturbation training types remains necessary for robust performance. \\

% We add the experiments to show that in-context learning actually can not fully address the schema evolution issues. In order to test whether the in-context learning can help address the schema evolution issue, we randomly select three examples (each example is a <NLQ, database schema after evolution, gold SQL after schema evolution> triple) as the demonstration in the prompt to help the models understand the schema after evolution. As Table \ref{tab:bird_human_eval} shows, compared with GPT-4 zero-shot (ZS) results, in-context learning (ICL) only largely exceeds zero-shot setting on ‘split columns’ type and is close to zero-shot setting for other perturbation types. This indicates that in-context learning is not always helpful for addressing
% the schema evolution problem. We hypothesize that it’s because the demonstration examples in the in-context learning can not cover all the cases of the schema change and SQL change, so for those test cases that are highly different with the demonstration examples, ICL can not bring benefit. But for ‘split columns’ types, since the column changes always bind to several types such as the name, address and date split, so the demonstration examples make ICL work better on this perturbation type. Table \ref{tab:bird_human_eval} shows that fine-tuning CodeLlama with perturbation training data achieves better results than in-context learning, which signals that fine-tuning is still needed. \\

\textbf{\#\#\# Revised Section}: \\

We add the human evaluation results for in-context learning in Table \ref{tab:bird_human_eval}. We add how we implement in-context learning in Section \ref{baselines} (Baselines). We add the results analysis in Section \ref{baseline_comparison}.


\noindent\rule{\linewidth}{0.5pt}


\textbf{\#\#\# Suggestion}: \\

May be Split / Merge would be another column-level operations for compound columns (E.g. address, date, etc.)? Column transformations? e.g. Birthday -> Age… Likewise column values changes would be another category all together? Eg. Fahrenheit -> Celsius, Category, classification, taxonomy changes, etc. Column value changes are particularly difficult ones to handle in real world text-to-sql applications. \\


\textbf{\#\#\# Response}: \\

Thanks for the wonderful suggestion! We add `split columns' and `merge columns' into our schema evolution taxonomy. They indeed make our taxonomy and experiments more complete. \\
For the column category change such as `Fahrenheit to Celsius', they all belong to temperature. If such change can reflect on the column name change, then our `column rename' type already covers such an evolution. But for the column value change, which only changes the value instead of the column name, we don't include it currently as it belongs to the database content change rather than the database schema change. It's out of the scope of our schema evolution problem. \\

\textbf{\#\#\# Revised Section}: \\

We add `split columns' and `merge columns' into our schema evolution taxonomy. We add Section \ref{data_collection_for_each_type} (Data Collection of Each Perturbation Type) and the data statistics of these two types in Table \ref{tab:data_stat_plus_manipulated_stat}. We add the experiment results for these two types in Table \ref{tab:bird_main_results2}, Table \ref{tab:bird_human_eval} and Table \ref{tab:bird_exec_acc}. Besides, we also revise our Figure \ref{fig:overview} and Figure \ref{fig:appendix_examples} to include these two schema evolution types.


}
\end{tcolorbox}
\end{figure*}




\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Reviewer 2 - Page 2}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer2}{blue color for reviewer 2}.\\


\textbf{\#\#\# Suggestion}: \\

Not sure what adding table that are irrelevant is going to improve text-to-sql. Shouldn’t the approach be to add tables that are at least in the same domain, potentially also relevant to the specific query such that the LLM can learn to pick the right tables to us in the SQL? Based on the results it seems there is a some improvement. Explanation on models tendency to join all tables is interesting. \\


\textbf{\#\#\# Response}: \\


Thank you for your thoughtful question. Our goal in adding irrelevant tables is to simulate real-world scenarios where databases often contain many tables unrelated to a given user query. In such settings, a robust text-to-SQL model must be able to identify and focus on the relevant subset of the schema while ignoring distracting or unrelated tables.

For example, in a university database with tables such as Students, Courses, and Enrollments, a user may ask: “What are the names of students enrolled in CS101?” Although the correct SQL query only involves the three aforementioned tables, the full schema may also include tables like DormRooms or CafeteriaMenus, which are unrelated to the question. In this case, the model is expected to ignore these irrelevant tables and still generate the correct SQL. Our perturbation ``add tables'' intentionally mimics this setting by introducing such extraneous tables, without changing the NLQ or the gold SQL, in order to evaluate the model’s ability to remain focused and accurate in the presence of schema distraction.



}
\end{tcolorbox}
\end{figure*}

==> reviewer3.tex <==
\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Reviewer 3 - Page 1}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer3}{green color for reviewer 3}.\\

\textbf{\#\#\# Suggestion}: \\

In Section 5, the authors evaluated 4 open-source LLMs and 2 closed-source LLMs. However, these models are base LLMs widely used across various downstream tasks (e.g., mathematics, coding) and are not NL2SQL-specific baseline models. State-of-the-art NL2SQL methods typically involve multiple sub-steps, including Schema Linking, which is designed to select a subset of relevant tables/columns from a database. This step is directly related to the evaluation goals of EvoSchema. Therefore, the authors should include evaluations with NL2SQL-specific baselines to improve the experimental setup and strengthen the effectiveness and generalizability of the conclusions.\\


\textbf{\#\#\# Response}: \\

Thanks for the wonderful suggestion! We include CHESS as our baseline. We apply the schema selection (SS) and candidate generation (CG) components developed in their work. For schema selection, we use advanced gpt-4o model to prune the database schema and remove the irrelevant tables and the irrelevant columns in the selected tables, so that we only input the most relevant tables and columns into the model for SQL generation. To ensure a fair comparison with our primary finetuning approach, we use a fine-tuned CodeLlama model trained without any schema perturbation data as the SQL generation (CG) model. This setup allows us to isolate and evaluate the effectiveness of a schema selection component in addressing schema evolution. \\


\textbf{\#\#\# Revised Section}: \\
We add the CHESS-SQL results on Table \ref{tab:bird_human_eval}. And we add how we implement CHESS in Section \ref{baselines} (Baselines). We add the results analysis in Section \ref{baseline_comparison}. \\

\noindent\rule{\linewidth}{0.5pt}

\textbf{\#\#\# Suggestion}: \\

Moreover, since NL2SQL is an end-to-end task, users are more concerned about whether the generated SQL accurately answers the user’s question, as reflected by the Execution Accuracy (EX) metric, rather than intermediate metrics like Table/Column Match F1. Although the authors mention EX in Section 5.2, only Table 4 in Section 6 provides EX results. Furthermore, the results in Table 4 indicate a decline in overall EX performance after training on perturbation-augmented datasets (despite improvements for some perturbation types). Therefore, the authors should include more comparisons using the EX metric in experiments (e.g., Table 3) and provide detailed analyses to help researchers understand EvoSchema’s impact on the end-to-end performance of NL2SQL tasks. Additionally, the authors should clarify which specific model was used in the experiment reported in Table 4. \\

\textbf{\#\#\# Response and Revised Section}: \\


We add Table \ref{tab:bird_exec_acc} to show the execution accuracy for all the LLMs (CodeLlama, Mistral, Llama3, SQLCoder, GPT-3.5 and GPT4) mentioned in Table \ref{tab:bird_main_results2} and add detailed analysis and underlying reasons in Section \ref{main_results} (Main Results). We also add human evaluation results in Table \ref{tab:bird_human_eval}. We would like to clarify that our experiments show improved average execution (EX) performance after training on perturbation-augmented data, with significant gains on challenging types such as split columns, add tables, and split tables. While there is a slight drop in EX for some minor perturbation types, we hypothesize that the training data is particularly beneficial for handling substantial schema changes, but may introduce minor noise in simpler cases where the model trained without perturbation data has already maximally learned the patterns. \\
% We want to clarify that our experiments show that EX performance is better on average after training on perturbation-augmented data and significantly better on splitting columns, adding and splitting tables, despite a slight drop for some perturbation types that has minor schema changes. We hypothesize that the perturbation train data is especially beneficial for handling substantial schema changes, but may introduce minor noise for simpler schema changes where fine-tuning without perturbation data has already maximum learned those schema. \\





}
\end{tcolorbox}
\end{figure*}



\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Reviewer 3 - Page 2}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer3}{green color for reviewer 3}.\\

\textbf{\#\#\# Suggestion}: \\

 In Section 6, the authors compare and analyze the results of multiple experiments but lack more intuitive comparative data. For example, in Section 6.1, the authors state that “Closed-source models are robust to different schema evolution types in general.” However, it is challenging for readers to clearly see this from Table 3. To improve the analysis, the authors should provide more intuitive statistical data (e.g., averages) to support their observations. Additionally, the authors should explore and reflect on the general underlying reasons behind the experimental phenomena, which would help researchers better understand the conclusions and contribute to further model improvements. \\


\textbf{\#\#\# Response}: \\

We add the MacroAvg, the arithmetic mean of Table Match F1, Column Match F1, Execution Accuracy and human evaluation across all perturbation types. The results can be seen in Table \ref{tab:bird_main_results2}, Table \ref{tab:bird_human_eval} and Table \ref{tab:bird_exec_acc}. We add detailed analysis and underlying reasons in Section \ref{main_results} (Main Results). 


When we state that “closed-source models are robust to different schema evolution types,” we refer to their relatively stable performance across perturbation types compared to the original non-evolved test set. In contrast, fine-tuned open-source models without perturbation training data exhibit significant performance drops—particularly on split columns, add tables, split tables, and merge tables—which introduce larger schema changes. We hypothesize that the stability and robustness of closed-source models stems from broader pretraining exposure and stronger internal schema reasoning capabilities, while the open-source models trained without perturbation types are more sensitive due to limited training on diverse schema variations. This motivates the need to fine-tune open-source models with perturbation training data to improve their generalization under schema evolution.
% For ``Closed-source models are robust to different schema evolution types in general'', we refer to that compared with original non-evolved test results, closed-sourced models' performance doesn't vary much across different perturbation types. But for fine-tuned open-sourced models, compared with original non-evolved test results, their performance drops a lot especially for ``split columns'', ``add tables'', ``split tables'' and ``merge tables'' perturbation types. These types will introduce relatively large perturbations which will have a higher impact for the fine-tuned open-sourced models (without perturbation training data). Closed-sourced models are more stable and more robust, we hypothesize that the robustness of closed-source models may stem from their broader pretraining exposure and stronger internal schema reasoning capabilities, while the more variable performance of open-source models may reflect their limited training on diverse schema structures. This is also why we need to fine-tune the open-sourced models with perturbation training data.
\\


\noindent\rule{\linewidth}{0.5pt}


\textbf{\#\#\# Suggestion}: \\


In Section 3.6, the authors propose various perturbation types, some of which, such as “Split Tables,” require additional manual verification and corrections (as shown in Figure 3). In real-world scenarios, the applicability of EvoSchema is directly influenced by the associated manual costs. Therefore, the authors should provide additional information on the manual effort required to ensure data quality when using LLMs to assist with specific perturbations on the BIRD dataset. This could include metrics such as the proportion of low-quality or erroneous data generated by LLMs that necessitate manual intervention. \\


\textbf{\#\#\# Response}: \\

Thanks for the suggestion! We add Cost Analysis in Section \ref{cost_analysis} (marked as green) to show the human verification cost and the LLM-synthesized low-quality data rate.
}
\end{tcolorbox}
\end{figure*}


==> tables/data_modification_stat.tex <==
\begin{table*}[ht]
\caption{Manipulation Statistics of perturbation data. ``Size" refers to ... ``Ratio" refers to...}

\small
\resizebox{1.0\linewidth}{!}{
\centering
\begin{tabular}{@{}l|cccc|cccc@{}}
\toprule
\multicolumn{9}{c}{Data Manipulation  Statistics (BIRD)} \\
\midrule
 \multirow{2}{*}{Perturbation Type} & \multicolumn{4}{c}{Size/Table}  & \multicolumn{4}{c}{Size/Query}  \\
 &Min & Mean & Median & Max &Min & Mean & Median & Max  \\
 \midrule
  & \multicolumn{8}{c}{Column Manipulation} \\
\midrule
Add Columns & 1 & 5.7 & 3 & 83 & 1 & 5.9 & 4 & 43\\
Remove Columns & 1 & 6.2 & 2 & 87 & 1 & 6.9 & 3 & 70 \\ 
Remove Col in SQL & 1 & 2.5 & 2 & 8 & 1 & 2.5 & 2.5 & 6 \\
Rename Columns &  1 & 4.3 & 3 & 46 & 1 & 4.4 & 3 & 46 \\ 
 \midrule
  & \multicolumn{8}{c}{Table Manipulation} \\
\midrule
Add Tables & - & - & - & - & 1 & 2 & 2 & 3    \\ 
Remove Tables & - & - & - & - & 1 & 1 & 1 & 1 \\
Rename Tables & - & - & - & - & 1 & 1.5 & 1 & 4  \\ 
Split Tables & - & - & - & - & 1 & 2.6 & 3 & 5 \\
Merge Tables & - & - & - & - & 2 & 2 & 2 & 2\\
 

\bottomrule
\end{tabular}
}
\label{tab:data_stat}
\end{table*}



==> tables/data_stat.tex <==
\begin{table}[hb]
\caption{Data statistics of original data and perturbation data. ``*": the evaluation data for calculating execution accuracy. We synthesize values to reconstruct the database after schema evolution, and filter out those not executable by gold SQL, which results in the smaller size of the evaluation data. \nop{Since we synthesize values to reconstruct the database after schema evolution, and it requires huge manual efforts to make the database executable by the new gold SQL after schema evolution of each instance, we filter out those not executable by new gold SQL, which results in the smaller size of the eval data.}}

\label{tab:data_stat}

\small
\resizebox{0.9\linewidth}{!}{
\centering
\begin{tabular}{@{}l|ccc@{}}
\toprule
\multicolumn{4}{c}{Data Statistics} \\
\midrule
 \multirow{2}{*}{Perturbation Type} & \multicolumn{3}{c}{BIRD}  \\
 &Train & Eval & Eval* \\
 \midrule
 Original & 9426 & 1534 & 789  \\
\midrule
Add Columns & 9219 & 1506 & 582  \\
Remove Columns &  9426 & 1534 & 773  \\ 
Remove Col in SQL & 9424 & 1534 & -  \\
Rename Columns & 9385 & 1533 & 674  \\ 
\midrule
Add Tables &  9387 & 1530 & 606  \\ 
Remove Tables & 7212 & 1171 & -  \\
Rename Tables &  9392 & 1534 & 735 \\ 
Split Tables & 9254 & 1515 & 178  \\
Merge Tables & 6930 & 1139 & 402 \\
 

\bottomrule
\end{tabular}
}
\end{table}



==> tables/minipage.tex <==
\begin{table}[t]
  \centering
  \begin{minipage}{0.46\linewidth}
    \centering
\caption{Intra-database Effect. This experiment emphasizes that the training and evaluation occur within the same database, instead of across databases.}
% \vspace{0.5\baselineskip}
\label{tab:intra_database_effect}
\small
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}l|cc|cc@{}}
\toprule
\multicolumn{5}{c}{Intra-database Effect} \\
\midrule
 \multirow{2}{*}{Perturbation Type} & \multicolumn{2}{c}{Table Match F1} & \multicolumn{2}{c}{Column Match F1} \\ 
 & w/o & w/ & w/o & w/\\
 \midrule
Original &  87.24 & \textbf{87.43} & 79.54 & \textbf{80.89}\\
\midrule
Add Columns & 87.14 & \textbf{87.43} & 76.36 & \textbf{78.92}\\
Remove Columns & \textbf{87.29} & 87.27 & 81.14 & \textbf{81.29} \\ 
Rename Columns & 85.71 & \textbf{86.43} & 77.45 & \textbf{79.09} \\ 
\midrule
Add Tables & 61.13 & \textbf{83.95} & 66.11 & \textbf{78.57}  \\ 
Remove Tables & - & - & - & -\\
Rename Tables & 86.33 & \textbf{86.67} & 79.44 & \textbf{79.96}\\ 
Split Tables & 71.82 & \textbf{78.52} & 75.09 & \textbf{77.42}  \\
Merge Tables & 85.11 & \textbf{87.44} & 71.43 & \textbf{74.72}\\
 

\bottomrule
\end{tabular}
}
\end{minipage}
\hfill
\begin{minipage}{0.46\linewidth}
    \centering
\caption{Evaluation on Spider. ``w/": the model is trained by merging the original data and all perturbation types; ``w/o": the model is only trained on the original training data.}
% \vspace{0.5\baselineskip}
\label{tab:spider_result}
\small
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}l|cc|cc@{}}
\toprule
\multicolumn{5}{c}{Spider Evaluation} \\
\midrule
 \multirow{2}{*}{Perturbation Type} & \multicolumn{2}{c}{Table Match F1} & \multicolumn{2}{c}{Column Match F1} \\
 & w/o & w/ & w/o & w/ \\
 \midrule
 Original & \textbf{99.72} & 99.65 & 90.54 & \textbf{91.35}\\
\midrule
Add Columns & \textbf{99.73} & 99.66 & 88.81 & \textbf{90.94}\\
Remove Columns &  99.35 & \textbf{99.65} & 86.13 & \textbf{88.59} \\ 
Rename Columns &  99.68 & \textbf{99.74} & 86.55 & \textbf{89.13}\\ 
\midrule
Add Tables &  62.46 & \textbf{98.80} & 66.49 & \textbf{90.54}\\ 
Remove Tables & - & - & - & - \\
Rename Tables & 99.24 & \textbf{99.25} & 89.71 & \textbf{90.99} \\ 
Split Tables &  73.27 & \textbf{90.24} & 76.76 & \textbf{86.93}\\
Merge Tables & 96.03 & \textbf{98.34} & 78.03 & \textbf{83.43}\\
 
 

\bottomrule
\end{tabular}
}
\end{minipage}
\end{table}


==> tables/minipage2.tex <==
\begin{table}[t]
  \centering
\begin{minipage}{0.33\linewidth}
    \centering
\caption{Evaluation on BIRD. ``w/": the model is trained with all the perturbation types; ``w/o": the model is only trained on the original training data.}
% \vspace{0.5\baselineskip}
\label{tab:bird_exec_acc}
\small
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}l|cc@{}}
\toprule
\multicolumn{3}{c}{Exec Acc on BIRD\nop{\tablefootnote{Since the schema evolution may lead to database restructure and there will be no existing values for the new database after schema change. We synthesize values to create new databases after schema evolution and execute the new gold SQLs after schema evolution on the new databases.}}} \\
\midrule
 \multirow{2}{*}{Perturbation Type} & \multicolumn{2}{c}{Exec Acc} \\
 & w/o & w/ \\
 \midrule
 Original &  \textbf{62.36} & 61.47 \\
\midrule
Add Columns & \textbf{60.99} & 60.31\\
Remove Columns & \textbf{62.61} & 60.67 \\ 
Rename Columns &  58.75 & \textbf{58.90}\\ 
\midrule
Add Tables & 49.50 & \textbf{62.54}\\ 
Remove Tables & - & - \\
Rename Tables & 58.64 & \textbf{59.05} \\ 
Split Tables & 50.00 & \textbf{60.67}  \\
Merge Tables & 48.76 & \textbf{52.88}\\
 
 

\bottomrule
\end{tabular}
}
\end{minipage}
\hfill
\begin{minipage}{0.65\linewidth}
\centering
\caption{Irrelevant tables effect. ``w/”: the model is trained with all the perturbation types; ``w/o”: the model is only trained on the original training data; ``w/o+": the model is only trained on the original training data, but for the input table schema, we also add irrelevant tables.}
% \vspace{0.5\baselineskip}
\label{tab:add_irrelevant_tables_effect}
\resizebox{1\linewidth}{!}{
\centering
\begin{tabular}{@{}l|ccc|ccc@{}}
\toprule
\multicolumn{7}{c}{Add Irrelevant Tables Effect} \\
\midrule
 \multirow{2}{*}{Perturbation Type} & \multicolumn{3}{c}{Table Match F1} & \multicolumn{3}{c}{Column Match F1} \\ 
 & w/o & w/o+ & w/ & w/o & w/o+ & w/\\
 \midrule
Original & 89.77 & 87.65 & \textbf{90.42} & 80.66 & 79.24 & \textbf{81.64} \\
\midrule
Add Columns & 89.73 & 86.35 & \textbf{90.27} & 78.26 & 75.31 & \textbf{80.27} \\
Remove Columns & 89.82 & 87.30 & \textbf{90.24} & 82.67 & 80.74 & \textbf{82.75}  \\ 
Rename Columns & \textbf{85.28} & 81.90 & 85.07 & 76.50 & 73.28 & \textbf{76.94}  \\ 
\midrule
Add Tables &  57.88 & 88.01 & \textbf{89.50} & 63.81 & 79.51 & \textbf{81.14}  \\ 
Remove Tables & - & - & - & - & - & -\\
Rename Tables & 88.84 & 86.84 & \textbf{90.32} & 79.60 & 78.47 & \textbf{80.91} \\ 
Split Tables &  71.99 & 67.27 & \textbf{81.55} & 75.30 & 70.39 & \textbf{78.45}  \\
Merge Tables & 87.52 & 85.36 & \textbf{88.95} & 67.73 & 65.78 & \textbf{68.98}\\
 

\bottomrule
\end{tabular}
}
\end{minipage}
\end{table}



% \vspace{-1em}



==> tables/more_baselines_and_human_eval.tex <==
\begin{table}[hb]
  \centering
\caption{Human Evaluation on \texttt{EvoSchema}. ``ZS'' refers to zero-shot, which prompts models without any examples. \textcolor{reviewer2}{``ICL'' refers to in-context learning, which prompts models with three demonstration examples.} ``w/o'' means fine-tuning model with perturbation training data; ``w/'' means fine-tuning model without perturbation training data. Bold color indicates the best performance among each row.}
% \vspace{0.5\baselineskip}
\label{tab:bird_human_eval}
\small
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{@{}l|ccccc@{}}
\toprule
\multicolumn{6}{c}{Human Evaluation on \texttt{EvoSchema}} \\
\midrule
 \multirow{2}{*}{Perturbation Type} & \multicolumn{2}{c}{GPT-4} & \multicolumn{2}{c}{Code Llama} & \textcolor{reviewer3}{CHESS$_{SS+CG}$}\\
 & ZS & \textcolor{reviewer2}{ICL} & w/o & w/\\
 \midrule
 Original &  70 & 62 & \textbf{72} & 70 & 68 \\
\midrule
Add Columns & 66 & 58 & 70 & 68 & \textbf{72}\\
Remove Columns & 72 & 66 & 70 & 68 & \textbf{72} \\ 
Rename Columns & 64 & 60 & 60 & 58 & \textbf{64} \\ 
\textcolor{reviewer2}{Split Columns} & 46 & 59 & 41 & \textbf{62} & 49\\
\textcolor{reviewer2}{Merge Columns} & 68 & 66 & 70 & \textbf{70} & 66 \\
\midrule
Add Tables & 60 & 60 & 52 & \textbf{66} & 60\\ 
Remove Tables & - & - & - & - & -\\
Rename Tables &  66 & 68 & \textbf{70} & 68 & 64 \\ 
Split Tables &  62 & 56 & 52 & \textbf{70} & 52 \\
Merge Tables & 60 & 62 & 58 & \textbf{68} & 54 \\
\midrule
\textcolor{reviewer3}{MacroAvg} & 63 & 62 & 61 & \textbf{67} & 62 \\
 
 

\bottomrule
\end{tabular}
}
\end{table}
